The mechanics of shuffle products and their siblings

We carry on the investigation initiated in [15] : we describe new shuffle products coming from some special functions and group them, along with other products encountered in the literature, in a class of products, which we name $\varphi$-shuffle products. Our paper is dedicated to a study of the latter class, from a combinatorial standpoint. We consider first how to extend Radford's theorem to the products in that class, then how to construct their bi-algebras. As some conditions are necessary do carry that out, we study them closely and simplify them so that they can be seen directly from the definition of the product. We eventually test these conditions on the products mentioned above.

==> macrosB.tex <==
%\usepackage[latin1]{inputenc}
%\usepackage[frenchb]{babel}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage{epic,eepic}
%\usepackage{graphicx}

\newcommand{\COMPLETER}[1]{$\cdots \cdots$ {\sc #1}}

% caligraphique
\newcommand{\calA}{{\mathcal A}}
\newcommand{\calZ}{{\mathcal Z}}
\newcommand{\calL}{{\mathcal L}}
\newcommand{\calM}{{\mathcal M}}
\newcommand{\calH}{{\mathcal H}}
\newcommand{\calC}{{\mathcal C}}
\newcommand{\calQ}{{\mathcal Q}}
\newcommand{\calS}{{\mathcal S}}

% Lettres gothiques
\def\g{\mathfrak{g}}

% Ensemble de nombres
\newcommand{\N}{{\mathbb N}}
\renewcommand{\P}{\N_{>0}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\K}{{\mathbb K}}

% Fonctions mathematiques
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}
\newcommand{\pref}[1]{(\ref{#1})}

\newcommand{\Frac}[2]{\displaystyle \frac{#1}{#2}}
\newcommand{\Sum}[2]{\displaystyle{\sum_{#1}^{#2}}}
\newcommand{\Prod}[2]{\displaystyle{\prod_{#1}^{#2}}}
\newcommand{\Int}[2]{\displaystyle{\int_{#1}^{#2}}}
\newcommand{\Lim}[1]{\displaystyle{\lim_{#1}\ }}

\newcommand{\eps}{{\varepsilon}}
\newcommand{\e}{{\epsilon}}
\newcommand{\into}{{\ \rightarrow\ }}
\newcommand{\mi}[1]{\mathbf{#1}}
\newcommand{\ok}{\tab $\Box$\bigskip}
\newcommand{\Var}{{\mathbb V}ar}

%apportHoang
\newcommand{\pathe}{{\rightsquigarrow}}
\def\pol#1{\langle #1 \rangle}
\def\Lyn{{\mathcal Lyn}}
\def\Lirr{{\mathcal L_{irr}}}
\def\llm#1{\mathcal #1}
\def\calCX{\calC \langle X \rangle}
\def\calCY{\calC \langle Y \rangle}
\def\CX{\C \langle X \rangle}
\def\CY{\C \langle Y \rangle}
\def\abs#1{|#1|}
\def\absv#1{\|#1\|}
\def\Conv{{\rm CV}}
\def\AXX{\serie{A}{X}}
% 10pt
 \def\shuffle{\mathop{_{^{\sqcup\!\sqcup}}}} 

\gdef\stuffle{\;% 
  \setlength{\unitlength}{0.0125cm}% 
  \begin{picture}(20,10)(220,580) 
  \thinlines 
  \put(220,592){\line( 0,-1){ 10}} 
  \put(220,582){\line( 1, 0){ 20}} 
  \put(240,582){\line( 0, 1){ 10}} 
  \put(230,592){\line( 0,-1){ 10}} 
  \put(225,587){\line( 1, 0){ 10}} 
  \end{picture}\; 
} 

\gdef\ctuffle{\;% 
  \setlength{\unitlength}{0.0125cm}% 
  \begin{picture}(20,10)(220,580) 
  \thinlines 
  \put(220,592){\line( 0,-1){ 10}} 
  \put(220,582){\line( 1, 0){ 20}} 
  \put(240,582){\line( 0, 1){ 10}} 
  %\put(230,592){\line( 0,-1){ 10}} 
  \put(225,587){\line( 1, 0){ 10}} 
  \end{picture}\; }


\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{example}{Example}
\newtheorem{question}{Question}
\newtheorem{remark}{Remark}
\newtheorem{proof}{Proof}
%\newtheorem{appendix}{APPENDIX}
% Fonctions mathematiques
%\newcommand{\1}{\operatorname{1}}
\newcommand{\Li}{\operatorname{Li}}
\newcommand{\ad}{\operatorname{ad}}
\renewcommand{\o}{\operatorname{o}}
\renewcommand{\O}{\operatorname{O}}
\newcommand{\Span}{\operatorname{span}}
\newcommand{\Lyndon}{\operatorname{Lyndon}}
\newcommand{\G}{\operatorname{G}}

\def\Sh{\mathrm{Sh}}
\def\LI{\mathrm{LI}}
\def\L{\mathrm{L}}
\def\H{\mathrm{H}}
\def\MZV{\ensuremath{\mathrm{MZV}}}
\def\Qsym{\mathrm{Qsym}}
\def\calHT{\mathcal{H}^\mathtt{0}}
\def\P{\mathrm{P}}
\def\Ng{\mathrm{N}}
\def\Zs{\mathrm{Z}}
\def\A{\mathrm{A}}
\def\Ann{\mathrm{Ann}}
\def\F{\mathrm{F}}
\def\G{\mathrm{G}}

\def\deg{\mathrm{deg}}
\def\wgt{\mathrm{wgt}}

\newcommand{\poly}[2]{#1 \langle #2 \rangle}
\def\ZX{\poly{\Z}{X}}
\def\QX{\poly{\Q}{X}}
\def\kX{\poly{\mathbb{k}}{X}}
\def\CX{\poly{\C}{X}}

\def\QY{\poly{\Q}{Y}}
\def\RY{\poly{\R}{Y}}
\def\CY{\poly{\C}{Y}}

\newcommand{\Stuffle}[2]{\big(\poly{#1}{#2},\stuffle\big)}

\newcommand{\serie}[2]{#1 \langle \! \langle #2 \rangle \! \rangle}
\def\AXX{\serie{A}{X}}
\def\AYY{\serie{A}{Y}}
\def\QYY{\serie{\Q}{Y}}
\def\KXX{\serie{\K}{X}}
\def\RXX{\serie{R}{X}}
\def\ZXX{\serie{\Z}{X}}
\def\QXX{\serie{\Q}{X}}
\def\CcXX{\serie{\C^{\mathrm{cont}}}{X}}
\def\QcXX{\serie{\Q^{\mathrm{cont}}}{X}}
\def\QratXX{\serie{\Q^{\mathrm{rat}}}{X}}
\def\ReXX{\serie{\R}{X}}
\def\CXX{\serie{\C}{X}}
\def\CYY{\serie{\C}{Y}}

\def\QY_0{\Q\left\langle{Y_0}\right\rangle}
\def\pol#1{\langle #1 \rangle}
\def\ser#1{\langle\!\langle #1 \rangle\!\rangle}
\def\AX{A \langle X \rangle}
\def\KX{\K \langle X \rangle}
\def\AY{A \langle Y \rangle}
\def\KY{\K \langle Y \rangle}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calT}{\mathcal{T}}

\def\FRX{\calF(\calR)\langle X \rangle}
\def\FRXX{\serie{\calF(\calR)}{X}}

\def\Lie{{\cal L}ie}
\def\LX{\Lie_{R} \langle X \rangle}
\def\LAX{\Lie_{A} \langle X \rangle}
\def\LAXX{\Lie_{A} \langle\!\langle X \rangle \!\rangle}
\def\LQX{\Lie_{\Q} \langle X \rangle}
\def\LQY{\Lie_{\Q} \langle Y \rangle}
\def\LKX{\Lie_{\K} \langle X \rangle}
\def\LQXX{\Lie_{\Q} \langle\!\langle X \rangle \!\rangle}
\def\LXX{\Lie_{\C} \langle\!\langle X \rangle \!\rangle}
\def\ShQX{\Sh_{\Q} \langle X \rangle}
\def\ShCX{\Sh_{\C} \langle X \rangle}

\def\mzero{{\mathfrak m}_0}
\def\mun{{\mathfrak m}_1}
\def\PKZ{\Phi_{KZ}}
\def\HR{\calH_\R}

\def\Axiom{{\sc Axiom}}
\def\Maple{{\sc Maple}}

%\newenvironment{proof}{\par \noindent {\sc Proof}\ --\ }{$\square$ \par}
%\newenvironment{remark}{\par \noindent {\sc Remark}\ --\ }{$\square$ \par}
%\newenvironment{example}
%	{\par \noindent {\sc Example}\ --\ }{$\square$ \par}

\newenvironment{myabstract}
	{\begin{quote} {\sc Abstract}\ --\ }
	{\end{quote}}

\newenvironment{system}
       {$$ \left\{ \begin{array}{lcll}} 
       {\end{array} \right. $$}
       
\def\CX{\C \langle X \rangle}
\def\CXX{\serie{\C}{X}}
 \newenvironment{varsystem}[1][]
       {\begin{eqnarray} #1 \left\{ \begin{array}{l@{}c@{}l}}
       {\end{array} \right. \end{eqnarray}}
 \newcommand{\calB}{{\cal B}}
\newcommand{\calR}{{\cal R}}
\newcommand{\LEx}{Lie exponential}
\newcommand{\LS}{Lie series }
\newcommand{\bs}{{\backslash}}
\newcommand{\ds}{\displaystyle}

\def\Lim{\displaystyle\lim}
\def\Sum{\displaystyle\sum}
\def\Prod{\displaystyle\prod}
\def\Frac{\displaystyle\frac}
\def\path{\rightsquigarrow}
\def\reg{\mathop\mathrm{reg}\nolimits}
\def\prv{\underline{\it Proof }: }
\def\resg{\triangleleft}
\def\resd{\triangleright}
\def\bv{\mid}
\def\bbv{\bv\!\bv}
\def\abs#1{\bv\!#1\!\bv}

\gdef\minishuffle{{\scriptstyle \shuffle}}  
\gdef\ministuffle{{\scriptstyle \stuffle}}  

\newcommand{\myover}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}
\newcommand{\mychoose}[2]{\genfrac{(}{)}{0pt}{}{#1}{#2}}

\def\rd{\triangleright}
\def\rg{\triangleleft}
\def\deg{\mathop\mathrm{deg}\nolimits}
\def\w{\mathop\mathrm{\omega}\nolimits}
\def\supp{\mathop\mathrm{supp}\nolimits}
\def\sgn{\mathop\mathrm{sgn}\nolimits}
\def\som{\mathop\mathrm{som}\nolimits}
\def\car{\mathop\mathrm{car}\nolimits}
\def\card{\mathop\mathrm{card}\nolimits}
\def\dbinom#1#2{{#1\choose#2}}
\def\binom#1#2{{#1\choose#2}}
\let\hs\hspace     

%%====================================================
%\definecolor{MyDarkBlue}{rgb}{0,0.08,0.4} 
%\def\tcdb#1{\textcolor{MyDarkBlue}{#1}} 
%\def\tcb#1{\textcolor{blue}{#1}} 
%\def\tcr#1{\textcolor{red}{#1}} 
%\def\tcg#1{\textcolor{green}{#1}} 
%%====================================================*

